Deep Unrolling of Lanczos-based Laplacian Eigensolver for Crop Classification in Satellite Images

Per-pixel crop classification in satellite images is an important pre-processing step in remote crop monitoring. Leveraging progress in signed graph signal processing, we build an interpretable and lightweight neural network for binary crop classification (e.g., corn versus non-corn) in two stages: i) learn a signed graph from data, and ii) unroll a Lanczos-based eigensolver to compute the eigenvector $\u_1$ associated with the smallest eigenvalue of a hybrid graph Laplacian $\cL$ for spectral clustering. Specifically, we first construct a near-balanced signed graph $\cG^s$, where signed edge weights $w_{i,j}\in(-1,1)$ are computed from learned feature distances $d_{i,j}$ via a hyperbolic tangent mapping. Given $\cG^s$, we estimate $\u_1$ by unrolling the Lanczos algorithm and use $\mathrm{sign}(\u_1)$ for binary classification. Mathematically, we develop a theorem establishing conditions under which $\u_1$ can be well approximated after finite Lanczos iterations. Motivated by this theorem, we relax the classical Lanczos orthogonality constraints during unrolling and optimize end-to-end classification performance while promoting the derived conditions for accurate eigenvector approximation. Experiments on real-world Harmonized Landsat-Sentinel imagery show classification performance comparable to state-of-the-art deep learning models while reducing parameters by up to two orders of magnitude.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


